Sequential Optimization of Speed, Thermal Load, and Power Split in Connected HEVs

The emergence of connected and automated vehicles (CAVs) provides an unprecedented opportunity to capitalize on these technologies well beyond their original designed intents. While abundant evidence has been accumulated showing substantial fuel economy improvement benefits achieved through advanced powertrain control, the implications of the CAV operation on power and thermal management have not been fully investigated. In this paper, in order to explore the opportunities for the coordination between the onboard thermal management and the power split control, we present a sequential optimization solution for eco-driving speed trajectory planning, air conditioning (A/C) thermal load planning (eco-cooling), and powertrain control in hybrid electric CAVs to evaluate the individual as well as the collective energy savings through proactive usage of traffic data for vehicle speed prediction. Simulation results over a real-world driving cycle show that compared to a baseline non-CAV, 11.9%, 14.2%, and 18.8% energy savings can be accumulated sequentially through speed, thermal load, and power split optimizations, respectively.

==> ACC2018Ref <==
 @article{bauer2014thermal,
  title={{Thermal and Energy Battery Management Optimization in Electric Vehicles Using Pontryagin's Maximum Principle}},
  author={Bauer, S. and Suchaneck, A. and Le{\'o}n, F.},
  journal={Journal of Power Sources},
  volume={246},
  pages={808--818},
  year={2014},
  publisher={Elsevier}
}

@inproceedings{masoudi2017mpc,
  title={{MPC-Based Battery Thermal Management Controller for Plug-in Hybrid Electric Vehicles}},
  author={Masoudi, Y. and Azad, N.},
  booktitle={American Control Conference},
  year={2017},
  note={{Seattle, WA, USA}}
}


@article{yuksel2012development,
title={{Development of a simulation model to analyze the effect of thermal management on battery life}},
author={Yuksel, T. and Michalek, J.},
Note={{SAE Technical Paper 2012-01-0671}},
year={2012}
}

@inproceedings{lofberg2004yalmip,
  title={{YALMIP: A Toolbox for Modeling and Optimization in MATLAB}},
  author={Lofberg, J.},
  booktitle={2004 IEEE Int. Symp. on Computer Aided Control Sys. Design},
year={2004},
note={{New Orleans, LA, USA}},
}

@article{wachter2006implementation,
  title={{On the Implementation of an Interior-Point Filter Line-Search Algorithm for Large-Scale Nonlinear Programming}},
  author={W{\"a}chter, A. and Biegler, L.},
  journal={Mathematical Programming},
  volume={106},
  number={1},
  pages={25--57},
  year={2006},
  publisher={Springer}
}

@article{zhang2011charge,
  title={{Charge-Depleting Control Strategies and Fuel Optimization of Blended-Mode Plug-in Hybrid Electric Vehicles}},
  author={Zhang, B. and Mi, C. and Zhang, M.},
  journal={IEEE Trans. on Vehicular Tech.},
  volume={60},
  number={4},
  pages={1516--1525},
  year={2011},
  publisher={IEEE}
}

@article{zhang2012analytical,
  title={{Analytical Approach for the Power Management of Blended-Mode Plug-in Hybrid Electric Vehicles}},
  author={Zhang, M. and Yang, Y. and Mi, C.},
  journal={IEEE Trans. on Vehicular Tech.},
  volume={61},
  number={4},
  pages={1554--1566},
  year={2012},
  publisher={IEEE}
}

@article{lim2017distance,
  title={{Distance-Based Ecological Driving Scheme Using a Two-Stage Hierarchy for Long-Term Optimization and Short-Term Adaptation}},
  author={Lim, H. and Su, W. and Mi, C.},
  journal={IEEE Trans. on Vehicular Tech.},
  volume={66},
  number={3},
  pages={1940--1949},
  year={2017},
  publisher={IEEE}
}

@article{halbach2010model,
  title={{Model Architecture, Methods, and Interfaces for Efficient Math-Based Design and Simulation of Automotive Control Systems}},
  author={Halbach, S. and Sharer, P. and Pagerit, S. and Rousseau, A. and Folkerts, C.},
Note={{SAE Technical Paper 2010-01-0241}},
year={2010}
}


@article{zolot2002thermal,
  title={{Thermal Evaluation of Toyota Prius Battery Pack}},
  author={Zolot, M. and Pesaran, A. and Mihalic, M.},
Note={{SAE Technical Paper 2002-01-1962}},
year={2002}
}



@inproceedings{sun2015integrating,
  title={{Integrating Traffic Velocity Data into Predictive Energy Management of Plug-in Hybrid Electric Vehicles}},
  author={Sun, C. and Sun, F. and Hu, X. and Hedrick, J. and Moura, S.},
  booktitle={ACC},
  year={2015},
  note={{Chicago, IL, USA}}
}

@article{lefort2013hierarchical,
  title={{Hierarchical Control Method Applied to Energy Management of a Residential House}},
  author={Lefort, A. and Bourdais, R. and Ansanay-Alex, G. and Gu{\'e}guen, H.},
  journal={Energy and Buildings},
  volume={64},
  pages={53--61},
  year={2013},
  publisher={Elsevier}
}


@article{herrera2010evaluation,
  title={{Evaluation of Traffic Data Obtained via GPS-Enabled Mobile Phones: The Mobile Century field experiment}},
author={Herrera, J. and Work, D. and Herring, R. and Ban, X. and Jacobson, Q. and Bayen, A.},
journal={Transportation Research Part C: Emerging Technologies},
  volume={18},
  number={4},
  pages={568--583},
  year={2010},
  publisher={Elsevier}
}

@inproceedings{masoudi2015battery,
  title={{Battery Thermal Management of Electric Vehicles: An Optimal Control Approach}},
  author={Masoudi, Y. and Mozaffari, A. and Azad, N.},
  booktitle={ASME Dynamic Systems and Control Conference},
 year={2015},
  note={{Columbus, OH, USA}}
}

@inproceedings{kim2014real,
  title={{Real-Time Battery Thermal Management for Electric Vehicles}},
  author={Kim, E. and Shin, K. and Lee, J.},
  booktitle={ACM/IEEE 5th Int. Conference on Cyber-Physical Systems},
  year={2014},
  note={Berlin, Germany}
}

@article{cominesi2018two,
  title={{A Two-Layer Stochastic Model Predictive Control Scheme for Microgrids}},
  author={Cominesi, S. and Farina, M. and Giulioni, L. and Picasso, B. and Scattolini, R.},
  journal={IEEE Trans. on Control Systems Technology},
  volume={26},
  number={1},
  pages={1--13},
  year={2018},
  publisher={IEEE}
}

@article{farina2018hierarchical,
  title={{A Hierarchical Multi-Rate MPC Scheme for Interconnected Systems}},
  author={Farina, M. and Zhang, X. and Scattolini, R.},
  journal={Automatica},
  volume={90},
  pages={38--46},
  year={2018},
  publisher={Elsevier}
}
 
 
@inproceedings{Kelman11,
  title={{Bilinear Model Predictive Control of a HVAC System Using Sequential Quadratic Programming}},
  author={Kelman, A. and Borrelli, F.},
  booktitle={Proc. of the 18th IFAC World Congress},
 year={2011},
  note={{Milano, Italy}}
}

@article{Bhatti97,
title={{A Critical Look at R-744 and R-134a Mobile Air Conditioning Systems}},
author={Bhatti, M.S.},
Note={{SAE Technical Paper 970527}},
year={1997}
}

@article{kiss2014comparison,
  title={{Comparison of the Accuracy and Speed of Transient Mobile A/C System Simulation Models}},
  author={Kiss, T. and Lustbader, J.},
  journal={SAE International Journal of Passenger Cars-Mechanical Systems},
  volume={7},
  number={2014-01-0669},
  pages={739--754},
  year={2014}
}

@article{Rugh2008,
  title={{Vehicle Ancillary Load Reduction Project Close-Out Report: An Overview of the Task and a Compilation of the Research Results}},
  author={Rugh, J. and Farrington, R.},
Note={{Technical Report, NREL/TP-540-42454}},
year={2008}
}


@article{jeffers2015climate,
title={{Climate Control Load Reduction Strategies for Electric Drive Vehicles in Warm Weather}},
author={Jeffers, M. and Chaney, L. and Rugh, J.},
Note={{SAE Technical Paper 2015-01-0355}},
year={2015}
}

@ONLINE{NRELwhitepaper,
title = {{NREL Works to Increase Electric Vehicle Efficiency Through Enhanced Thermal Management}},
month = {June},
year = {2014},
url = {https://www.nrel.gov/docs/fy14osti/62241.pdf}
}

@incollection{zhang2016modeling,
  title={{Modeling Air Conditioning System with Storage Evaporator for Vehicle Energy Management}},
  author={Zhang, Q. and Canova, M.},
  booktitle={Automotive Air Conditioning},
  pages={247--266},
  year={2016},
  publisher={Springer}
}

@inproceedings{hwang2018,
  title={{Model Predictive Climate Control of Connected and Automated Vehicles for Improved Energy Efficiency}},
  author={Wang, H. and Kolmanovsky, I. and Amini, M. and Sun, J.},
  booktitle={ACC},
  year={2018},
note={{Milwaukee, WI, USA}}
}

@article{kiss2013new,
  title={{New Automotive Air Conditioning System Simulation Tool Developed in MATLAB/Simulink}},
  author={Kiss, T. and Chaney, L. and Meyer, J.},
  note={{SAE Technical Paper 2013-01-0850}},
  year={2013}
}

@article{rostiti2015rule,
  title={{A Rule-based Control for Fuel-efficient Automotive Air Conditioning Systems}},
  author={Rostiti, C. and Stockar, S. and Canova, M.},
  note={{SAE Technical Paper 2015-01-0366}},
  year={2015}
}

@inproceedings{tao2014cooling,
  title={{Cooling Air Temperature and Mass Flow Rate Control for Hybrid Electric Vehicle Battery Thermal Management}},
  author={Tao, X. and Wagner, J.},
  booktitle={ASME 2014 Dynamic Systems and Control Conference},
  year={2014},
 note={{San Antonio, TX, USA}}
 }
 
 @article{tao2015hybrid,
  title={{A Hybrid Electric Vehicle Thermal Management System - Nonlinear Controller Design}},
  author={Tao, X. and Zhou, K. and Ivanco, A. and Wagner, J. and Hofmann, H. and Filipi, Z.},
  note={{SAE Technical Paper  2015-01-1710}},
  year={2015}
}

@article{guanetti2018control,
  title={{Control of Connected and Automated Vehicles: State of the Art and Future Challenges}},
  author={Guanetti, J. and Kim, Y. and Borrelli, F.},
  journal={Annual Reviews in Control},
  volume={45},
  pages={18--40},
  year={2018},
  publisher={Elsevier}
}

@inproceedings{AminiCDC18,
  title={{Two-Layer Model Predictive Battery Thermal and Energy Management Optimization for Connected and Automated Electric Vehicles}},
  author={Amini, M.R. and Kolmanovsky, I. and Sun, J.},
  booktitle={57th IEEE CDC},
  year={2018},
note={{Miami Beach, FL, USA}}
}

@article{ptv2016ptv,
  title={{PTV VISSIM 9.0 User Manual}},
  author={PTV Group and others},
  journal={PTV AG, Karlsruhe, Germany},
  year={2016}
}

@article{wu2011shockwave,
  title={{A Shockwave Profile Model for Traffic Flow on Congested Urban Arterials}},
  author={Wu, X. and Liu, H. X.},
  journal={Transportation Research Part B: Methodological},
  volume={45},
  number={10},
  pages={1768--1786},
  year={2011},
  publisher={Elsevier}
}

@article{Zhen2018Traj,
  title={{Eco-trajectory Planning with Consideration of Queue Along Congested Corridor for Hybrid Electric Vehicles}},
  author={Yang, Z. and Feng, Y. and Gong, X. and Zhao, D. and Sun, J. },
  journal={Transportation Research Record},
  year={2019},
}

@inproceedings{barth2011dynamic,
  title={{Dynamic ECO-driving for Arterial Corridors}},
  author={Barth, M. and Mandava, S. and Boriboonsomsin, K. and Xia, H.},
  booktitle={2011 IEEE Forum on Integrated and Sustainable Transportation System},
  year={2011},
  note={{Vienna, Austria}}
}

@article{barth2009energy,
  title={{Energy and Emissions Impacts of a Freeway-Based Dynamic Eco-Driving System}},
  author={Barth, M. and Boriboonsomsin, K.},
  journal={Transportation Research Part D: Transport and Environment},
  volume={14},
  number={6},
  pages={400--410},
  year={2009},
  publisher={Elsevier}
}

@article{sciarretta2015optimal,
  title={{Optimal Ecodriving Control: Energy-Efficient Driving of Road Vehicles as an Optimal Control Problem}},
  author={Sciarretta, A. and De Nunzio, G. and Ojeda, L.},
  journal={IEEE Control Systems},
  volume={35},
  number={5},
  pages={71--90},
  year={2015},
  publisher={IEEE}
}

@inproceedings{prakash2016assessing,
  title={{Assessing Fuel Economy from Automated Driving: Influence of Preview and Velocity Constraints}},
  author={Prakash, N. and Cimini, G. and Stefanopoulou, A. and Brusstar, M.},
  booktitle={DSCC},
 year={2016},
  note={{Minneapolis, MN, USA}}
}

==> HEV_BTMModel.tex <==
\vspace{-0.1cm}
\section{Battery Thermal and Electrical Models} \label{sec:1}
%\vspace{-0.1cm}
%
To formulate an MPC for BTM system, both the electrical and thermal characteristics of the battery have to be captured by the prediction model. The thermal sub-model approximates the battery pack as a lumped mass ($m_{bat}$) with heat capacity $C_{th, bat}$, and can be described as follows~\cite{bauer2014thermal}:
%
\vspace{-0.15cm}
\begin{gather}
\label{eqn:Eq1}
\dot{T}_{bat}(t)=\frac{1}{m_{bat} C_{th,bat}}(I_{bat}^2R_{bat}+\dot{Q}),
\end{gather}
%
where, $T_{bat}$, $I_{bat}$, and $R_{bat}$ are the battery temperature, current, and internal resistance, respectively. $\dot{Q}<0$ is the required heat flow rate for cooling the battery, and it is treated as the input to the battery thermal model in this paper. %In practice, $\dot{Q}$ is provided through a combination of air and liquid cooling loops in electric vehicles. The liquid cooling consist of an electric A/C compressor and a coolant loop. The air cooling regulates the battery temperature by blowing the compartment air into the battery pack using a fixed or variable speed fan. Since the compartment air is cooled by the A/C compressor, the battery air cooling loop is also coupled to the vehicle HVAC system.

The electric system sub-model of the battery includes the battery voltage ($U_{bat}$), which can be expressed as a function of the open-circuit voltage ($U_{oc}$), $R_{bat}$, and $I_{bat}$ as follows:  \vspace{-0.2cm}
%
\begin{gather}
\label{eqn:Eq2}
U_{bat}=U_{oc}-I_{bat}R_{bat}
\end{gather}
%
$U_{oc}$ and $R_{bat}$ in (\ref{eqn:Eq2}) are functions of the battery state-of-charge ($SOC$) and $T_{bat}$. The battery current can be written as a function of the total demanded power as follows:  \vspace{-0.2cm}
%
\begin{gather}
\label{eqn:Eq3}
I_{bat}=({P_{trac}+P_{temp}})/{U_{bat}},
\end{gather}
%
where, $P_{trac}$ is the demanded traction power, and $P_{temp}$ is the required power to provide $\dot{Q}$ for the BTM system. It is assumed in Eq.~(\ref{eqn:Eq3}) that $P_{trac}$ and $P_{temp}$ are the main power loads on the battery, and other auxiliary loads on the battery are neglected. By substituting $U_{bat}$ in~(\ref{eqn:Eq2}) with $(P_{trac}+P_{temp})/I_{bat}$ (Eq.~(\ref{eqn:Eq3})), $I_{bat}$ can be re-written: \vspace{-0.35cm}

\small
\begin{gather}
\label{eqn:Eq4}
I_{bat}(t)=\frac{U_{oc}-\sqrt{U_{oc}^2-4R_{bat}(P_{trac}+P_{temp})}}{2R_{bat}}
\end{gather}
\normalsize

%
Using (\ref{eqn:Eq4}), Eq.~(\ref{eqn:Eq1}) becomes: \vspace{-0.15cm}
%
\begin{gather}
\label{eqn:Eq6}
\dot{T}_{bat}(t)=\frac{\frac{(U_{oc}-\sqrt{U_{oc}^2-4R_{bat}P_{trac}+P_{temp}})^2}{4R_{bat}}+\dot{Q}}{C_{th,bat}}.
\end{gather}
%
Moreover, $SOC$ is governed by: \vspace{-0.2cm}
%
\begin{gather}
\label{eqn:Eq5}
\dot{SOC}(t)=-\frac{I_{bat}}{C_{nom}}
\end{gather}
%
where, $C_{nom}$ is the nominal capacity of the battery. The demanded traction power can be estimated as~\cite{bauer2014thermal}:
%
\begin{gather}
\label{eqn:Eq7}
P_{trac}=\begin{cases}
\frac{V_{veh}(F_r+F_a+m\dot{V}_{veh}^2)}{\eta},~~~propelling\\
{V_{veh}(F_r+F_a+m\dot{V}_{veh}^2)}{\eta},~~~braking
\end{cases}
\end{gather}
%
where $V_{veh}$ and $m$ are the vehicle speed and mass. $\eta=\eta(\tau,\omega)$ is the traction system efficiency, which is a function of the torque ($\tau$) and the rotation speed ($\omega$) of the electric motor, and it is calculated by using a look-up table. $F_r$  and $F_a$ are rolling and aerodynamic resistances calculated as follows: \vspace{-0.5cm}
%
\begin{gather}
\label{eqn:Eq7_2}
F_r=C_rmg,\\
F_a=0.5\rho A_{f}C_dV_{veh}^2,
\end{gather}
%
with $C_r$ and $C_d$ being the rolling resistance and aerodynamic drag coefficients, $A_f$ the vehicle frontal area, and $\rho$ the air density. In this paper, the road is assumed to be plain, i.e., the road grade is zero. $P_{temp}$ is modeled as a linear function of the heat flow rate ${\dot{Q}}$~\cite{bauer2014thermal}: \vspace{-0.2cm}
%
\begin{gather}
\label{eqn:Eq8}
P_{temp}(\dot{Q})=a_c\dot{Q},~~\dot{Q}\leq 0,~~a_c<0
\end{gather}
%
where $a_c$ is a constant. The parameters of the battery and vehicle longitudinal dynamics are adopted from the Autonomie~\cite{halbach2010model} software library for an electric vehicle. These parameters are listed in Appendix~\ref{FirstAppendix}. Moreover, the high-fidelity thermal and electrical models of the battery, along with $R_{bat}(SOC,T_{bat})$, $U_{oc}(SOC,T_{bat})$, and $\eta(\omega,\tau)$ look-up tables are adopted from Autonomie, and will be used as the virtual testbed to carry out the simulations. \vspace{-0.1cm}

\section{Single-Layer MPC for Battery Thermal and Power Management}\label{sec:3} \vspace{-0.1cm}
%
The traditional BTM system attempts to maintain the battery temperature at a specified level, without considering the traffic information. A setpoint within the optimal temperature range of the battery operation is selected and tracked. Since the battery temperature can increase rapidly due to aggressive vehicle acceleration and deceleration, the desired battery temperature setpoint ($T_{bat}^{s.p.}$) is usually selected well below the upper limit of the optimum operation range to assure that the temperature stays within the limit during transients. This tracking approach, however, is conservative and designed for worst case scenarios without predictive traffic information. It often leads to considerable extra energy consumed for battery cooling. To exploit the traffic information made available through CAVs, and to improve thermal efficiency, a model predictive controller in an economy scheme is designed in this section to minimize the required battery cooling power, and maintain the battery temperature within the desired operation range. 

In order to formulate the MPC, first the thermal and electric models (Eqs.~(\ref{eqn:Eq5}) and (\ref{eqn:Eq6})) are discretized by applying the Euler forward method: \vspace{-0.5cm}
% f_{SOC}(k) f_{T_{bat}}(k)

\small
\begin{gather}
\label{eqn:Eq9}
SOC(k+1)=SOC(k)-~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~\\
T_s\Big(\frac{U_{oc}-\sqrt{U_{oc}^2-4R_{bat}(P_{trac}+P_{temp})}}{2C_{nom}R_{bat}}\Big), \nonumber
\end{gather}
%
\begin{gather}
\label{eqn:Eq10}
{T}_{bat}(k+1)={T}_{bat}(k)+~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~\\
T_s\Big(\frac{\frac{(U_{oc}-\sqrt{U_{oc}^2-4R_{bat}P_{trac}+P_{temp}})^2}{4R_{bat}}+\dot{Q}}{C_{th,bat}}\Big), \nonumber
\end{gather}
\normalsize
%
where, $T_s$ is the sampling time for control update (e.g., $T_s$=1~sec). We consider a single-layer MPC with an economy cost function formulated over a finite-time horizon ($N$) with $\dot{Q}$ being the optimization variable: \vspace{-0.15cm}
%-------------------------------------
\begin{gather} \label{eqn:Eq11}
\begin{aligned}
& \underset{\dot{Q}(\cdot|k)}{\text{min}} & & \sum_{i=0}^{N} P_{temp}(i|k), \\
% \end{aligned}
% \end{gather}
% %
% \begin{gather} \label{eqn:Eq11}
% \begin{aligned}
%\tilde{\boldsymbol{y}}(k) & \\
& \text{s.t.}
& & T_{bat}(i+1|k)=f_{T_{bat}}(i|k),~{i=0,\cdots,N},\\
& 
& & SOC(i+1|k)=f_{SOC}(i|k),~{i=0,\cdots,N},\\
& 
& &T_{bat}^{LL}\leq T_{bat}(i|k)\leq T_{bat}^{UL},~{i=0,\cdots,N},\\
& 
& &30\% \leq SOC(i|k)\leq 90\%,~{i=0,\cdots,N},\\
& 
& &-50~W\leq \dot{Q}(i|k)\leq 0,~{i=0,\cdots,N-1},\\
& 
& & T_{bat}(0|k)=T_{bat}(k),~SOC(0|k)=SOC(k),%\\
%& 
%& & \dot{Q}(0|k)=\dot{Q}(k)
\end{aligned}
\end{gather}
%-------------------------------------
%
{where, $(i|k)$ designates the prediction for the time instant $k+iT_s$ made at the time instant $k$.} The nonlinear MPC optimization problem (\ref{eqn:Eq11}) attempts to minimize the power spent for battery thermal managment $P_{temp}=a_c\dot{Q}$ over the prediction horizon, while enforcing the state and input constraints. $T_{bat}^{UL}$ and $T_{bat}^{LL}$ are the upper and lower limits of the battery operating temperature, and they are set to $40^oC$ and $20^oC$, respectively. Note that $\dot{Q}$ is always negative for battery cooling scenario. $f_{SOC}(k)$ and $f_{T_{bat}}(k)$ are the discritized nonlinear dynamics of $SOC$ and $T_{bat}$ calculated according to (\ref{eqn:Eq9}) and (\ref{eqn:Eq10}). The optimization problem is solved at every time step, then the horizon is shifted by one step ($T_s$), and only the current control is commanded to the system ($\dot{Q}(k)$). The MPC simulation is carried out on a desktop computer, with an Intel\textsuperscript{\textregistered} Core i7@2.60 GHz processor, in MATLAB\textsuperscript{\textregistered}/SIMULINK\textsuperscript{\textregistered} using YALMIP~\cite{lofberg2004yalmip} for formulating the optimization problem, and IPOPT\cite{wachter2006implementation} for solving the optimization problem numerically. 

Intuitively, the solution of the optimization problem in (\ref{eqn:Eq11}) results in the battery temperature to be as close as possible to the upper limit $T_{bat}^{UL}$, as it is equivalent to the minimum cooling power consumption. However, since sudden changes in the $P_{trac}$ could increase the battery temperature and cause $T_{bat}$ to exceed the desired range, MPC with different prediction horizons will respond differently. Fig.~\ref{fig:UDDS_T_bat_SingleLayer_MPC_LongH_resize} shows the results of applying the nonlinear MPC (\ref{eqn:Eq11}) with different prediction horizons ($N$) on the EPA Urban Dynamometer Driving Schedule (UDDS), where it is assumed that the entire driving cycle is available, and the battery initial temperature ($T_{bat,0}$) is the same in all the simulated runs. % for all scenarios, and $T_{bat}^{UL}$ is fixed, and set to be $40^oC$~\cite{zolot2002thermal}. 
Additionally, the MPC simulation results are compared with simple rule-based (On/Off) controller which attempts to maintain $T_{bat}$ at a constant level of $T_{bat}^{s.p.}$=$35^oC$. This setpoint is selected according to the setpoint given by the Autonomie software's BTM system~\cite{halbach2010model}.  %\vspace{-0.35cm}
%
\begin{figure}[h!]
	\begin{center}
		\includegraphics[width=6.85cm]{Results/UDDS_T_bat_SingleLayer_MPC_Modified_Final_V2_1.eps}  %\vspace{-0.75cm} 
        \includegraphics[width=6.85cm]{Results/UDDS_T_bat_SingleLayer_MPC_Modified_Final_V2_2.eps} \vspace{-0.3cm}   % The printed column width is 8.4 cm.
		\caption{The performance of the single layer MPC for battery thermal (top) and energy (bottom) management with different prediction horizons at $T_{bat,0}=35^oC$ for UDDS.}\vspace{-0.75cm} 
		\label{fig:UDDS_T_bat_SingleLayer_MPC_LongH_resize} 
	\end{center}
\end{figure}
%

Fig.~\ref{fig:UDDS_T_bat_SingleLayer_MPC_LongH_resize} shows that with a short prediction horizon ($N=10$), the controller does not have enough lead time to take mitigating actions to prevent constraint violation caused by sudden increase in the traction power around $t=200~sec$. However, as the prediction horizon is being extended, the MPC takes proactive actions to reduce the temperature before the heating load increases around $200~sec$, therefore significantly reducing the time for the battery to stay in over-temperature condition.~
%when the prediction horizon is $N=10$, the major rise in the demanded traction power around $t=200~sec$ becomes detectable to the MPC late. Thus, during the early seconds, the MPC minimizes the tempering power which leads to the increase in $T_{bat}$. Once the major rise in the traction power occurs, the battery temperature increases sharply, which leads the battery temperature hits $44^oC$. Eventually, when the battery is cooled down to below $T_{bat}^{UL}$, it will remain at $40^oC$ until the end of the driving cycle. 
Table~\ref{tab:Energy_Comparison} summarizes the results of single-layer MPC, in terms of energy saving and battery constraint violation, with the rule-based controller performance as the baseline. Compared to the simple rule-based controller, $4.5-5.3\%$ improvement in the energy consumption can be achieved by using the predictive controllers. The temperature upper limit violation, as expected, becomes less frequent as the prediction horizon being extended. It can be seen that when the horizon is longer than 120 $sec$, the MPC puts the efforts to decrease $T_{bat}$ from the early seconds, which eventually results in both fuel saving ($>5\%$) and reduced constraint violation. \vspace{-0.25cm}% violation. up to 41\% reduction in $T_{bat}^{UL}$ violation, while up to 5\% saving in the energy consumption can be achieved. 

%It should be mention that an add-on logic has been applied to the single-Layer MPC to avoid infeasibility when the temperature constraint is violated. 
%\linespread{1.3}
\begin{table}[h!]
\begin{center}
\small
\centering
\caption{Energy saving and battery constraint violation comparison of the Single-Layer MPC with different $N$ for Fig.~\ref{fig:UDDS_T_bat_SingleLayer_MPC_LongH_resize}. 
\label{tab:Energy_Comparison}} %\vspace{0.4cm}
\begin{tabular}{lcc}
        \hline\hline
~~~~~~~~~~$controller$& $SOC$ (\%) & $T_{bat}^{UL}$ Violation (sec)  \\ \hline
Rule-Based      & -~\textcolor{blue}{(Baseline)} & 101~\textcolor{blue}{(Baseline)}  \\ \hline
MPC~$N=10$ & \textcolor{blue}{$+$4.8\%} & 321~\textcolor{red}{($\uparrow$218\%)} \\\hline
%
MPC~$N=60$ & \textcolor{blue}{$+$4.5\%} & 225~\textcolor{red}{$(\uparrow$123\%)} \\
\hline
%
MPC~$N=120$ & \textcolor{blue}{$+$5.3\%} & 78~\textcolor{black!30!green}{($\downarrow$23\%)} \\
\hline
%
MPC~$N=180$ & \textcolor{blue}{$+$5.0\%} & 60~\textcolor{black!30!green}{($\downarrow$41\%)} \\
%
% $~~~max~CPU$      &  &  &  &  \\
% $time/iteration~[sec]$ & 2.40 & 4.51 & 9.57 & 18.47 \\
        \hline\hline
    \end{tabular}
\end{center} \vspace{-0.6cm} 
\end{table}
\linespread{1}

This study confirms the advantages of incorporating the future traffic information for battery thermal and energy optimization via an MPC framework. Due to the large thermal inertia and therefore large time constant in the thermal response, however, BTM system requires much longer horizon information to capitalize on the benefits associated with the MPC approach. %It was concluded that availability of information of future events helps to maintain the temperature within the desired range, and enhance the final state-of-charge of the battery. 
%While the results of the battery energy management ($SOC$) are almost the same for different prediction horizons, as $N$ becomes longer, the battery thermal behavior significantly changes, and the violation of the battery temperature operation limit reduces. This observation can be explained with respect to the difference in the time constants of the battery thermal and electrical systems. Compared to power management systems of the EVs, which deal with a relatively fast dynamic, and is usually performs in a short control horizon, it can be seen that the BTM system requires much longer horizon information. %This is because of the thermal inertia of the BTM system which makes the thermal dynamic relatively slow. Thus, the BTM systems require a much longer time horizon.  

On the other hand, the implementation of the MPC over a long horizon is not practical for two main reasons: (i) it is computationally demanding, and (ii) the accuracy in future traffic event prediction over a longer horizon is poor. The average %and maximum 
computation time per iteration for the {single-layer} MPC with different prediction horizons is listed in Table~\ref{tab:Computation Time Comparison}. It can be seen from Table~\ref{tab:Computation Time Comparison} that the MPC with a long horizon is computationally expensive with average computation time exceeding the sampling time $T_s=1~sec$. This clearly impedes the real-time implementation of the single-layer MPC. Moreover, vehicle speed profile can be accurately estimated using traffic and infrastructure information (V2I/V2X) only over a short horizon~\cite{sun2015integrating}. The prediction of the vehicle speed over an extended horizon is subject to uncertainties, which consequently affects the performance of the MPC for BTM over a long horizon. The issue with computation complexity and information availability motivate us to seek the alternative control solution presented in Sections~\ref{sec:TrafficFlow} and \ref{sec:TwoMPC}.  \vspace{-0.4cm} 
%
%\linespread{1.3}
\begin{table}[h!]
\begin{center}
\small
\centering
\caption{Computation time comparison of the Single-Layer MPC with different prediction horizon for the results shown in Fig.~\ref{fig:UDDS_T_bat_SingleLayer_MPC_LongH_resize}. 
\label{tab:Computation Time Comparison}} %\vspace{0.4cm}
\begin{tabular}{lcccc}
        \hline\hline
~~~~~~~~~~$N$& 10 & 60 & 120 & 180 \\ \hline
$~~~average~CPU$      & 0.75 & 2.22 & 6.24 & 10.78 \\
$time/iteration~[sec]$ & \textcolor{red}{-} & \textcolor{red}{$\uparrow$196\%} & \textcolor{red}{$\uparrow$732\%} &  \textcolor{red}{$\uparrow$1337\%}\\%\hline
%
% $~~~max~CPU$      &  &  &  &  \\
% $time/iteration~[sec]$ & 2.40 & 4.51 & 9.57 & 18.47 \\
        \hline\hline
    \end{tabular}
\end{center} \vspace{-0.5cm} 
\end{table}
\linespread{1}

\vspace{-0.25cm} 
\section{Traffic Flow Model for Long Horizon Prediction} \label{sec:TrafficFlow}
%
As discussed in Section~\ref{sec:3}, the information about future driving conditions, in particular, the vehicle speed profile over a long horizon, can facilitate the design of an energy-efficient BTM system. We show in this section that an approximate knowledge of future vehicle speed profile can be based on the average traffic flow velocity ($V_{flow}$) estimate according to the approach proposed in~\cite{sun2015integrating}. This knowledge, when integrated into single-layer MPC controller, can reduce energy consumption.~%While an exact demanded traction power over a short horizon is essential for the energy management of the electrified vehicles, it will be shown in this section that a minimum knowledge of the traffic flow information over a long horizon can be beneficial for BTM system optimization. Here, the demanded traction power of the vehicle over a long horizon is estimated with respect to the average traffic flow velocity ($V_{flow}$) according to the approach proposed in~\cite{sun2015integrating}. 

In~\cite{sun2015integrating}, the traffic flow data are extracted from a traffic monitoring system described in~\cite{herrera2010evaluation}, based on GPS-enabled smartphones. This system exploits the extensive coverage of the cellular network, GPS-based position and velocity measurements, and the communication infrastructure of cellphones. In this paper, we assume that the traffic flow data are being collected, analyzed, and updated by a central/cloud server in real-time, and they are available to the vehicle control system at no extra computational cost. Additionally, $V_{flow}$ is updated every cycle as the traffic flow condition changes in the downstream. Fig.~\ref{fig:NYCC_Estimate} illustrates the concept of the average traffic flow speed trajectory and compares it against the actual speed profile. As can be observed, the long-horizon prediction of the vehicle speed profile is close to the actual vehicle speed for the first few cycles. Then, the predicted vehicle speed merges into the traffic flow average speed band (the gray band in Fig.~\ref{fig:NYCC_Estimate}) over the long horizon. For more details, see~\cite{sun2015integrating}. \vspace{-0.3cm} 
%
\begin{figure}[h!]
	\begin{center}
		\includegraphics[width=8.5 cm]{Results/NYCC_Estimate_V3.eps} \vspace{-0.45cm}   % The printed column width is 8.4 cm.
		\caption{The virtual traffic flow speed versus the actual driving cycle. In this paper, it is assumed that the traffic flow velocity information is repeatedly updated every cycle over a 250-$sec$ window. }\vspace{-0.65cm} 
		\label{fig:NYCC_Estimate} 
	\end{center}
\end{figure}
%%
\begin{figure*}
	\begin{center}
		\includegraphics[scale=0.43]{Results/UDDS_T_bat_LongH_SingleLayer_SecondLayer_180.eps} \vspace{-0.3cm}   % The printed column width is 8.4 cm.
		\caption{The performance of the Single-Layer and Two-Layer MPCs with accurate and estimated vehicle speed profiles over a long horizon for UDDS.}\vspace{-0.75cm} 
		\label{fig:UDDS_T_bat_LongH_SingleLayer_SecondLayer_180} 
	\end{center}
\end{figure*}
%

% \newcommand{\greenline}{\raisebox{2pt}{\tikz{\draw[-,black!30!green,solid,line width = 0.9pt](0,0) -- (3mm,0);}}}
%
\newcommand{\greenline}{\raisebox{2pt}{\tikz{\draw[-,green,solid,line width = 0.9pt](0,0) -- (3mm,0);}}}
%
\newcommand{\blueline}{\raisebox{2pt}{\tikz{\draw[-,black!30!blue,solid,line width = 0.9pt](0,0) -- (3mm,0);}}}
%
\newcommand{\redline}{\raisebox{2pt}{\tikz{\draw[-,red,dashed,line width = 1.5pt](0,0) -- (4.5mm,0);}}}
%
\newcommand{\bluearrow}{\raisebox{2pt}{\tikz{\draw[->,blue,solid,line width = 1.5pt](0,0) -- (5mm,0);}}}
%
\newcommand{\rectangle}{\raisebox{0pt}{\tikz{\draw[black,solid,line width = 1.0pt](2.mm,0) rectangle (3.5mm,1.5mm);\draw[-,black,solid,line width = 1.0pt](0.,0.8mm) -- (5.5mm,0.8mm)}}}

%\vspace{-0.25cm} 
To understand the effects of uncertainties associated with the long prediction horizon, we consider the implementation of the single-layer MPC with both the actual speed profile, and with the one estimated from the traffic flow information. Fig.~\ref{fig:UDDS_T_bat_LongH_SingleLayer_SecondLayer_180} shows the results of evaluating the single-layer MPC (Eq.~(\ref{eqn:Eq11})) with a long horizon ($N=180~sec$) and with the exact speed profile and with the speed profile extracted from traffic flow information,  together with results of the on/off rule-based controller as the baseline.~% , and the single-layer MPC results from Fig.~\ref{fig:UDDS_T_bat_SingleLayer_MPC_LongH_resize} with the prediction horizon $N=180~sec$.~%Despite the mismatch between the real vehicle speed profile and vehicle speed profile based on the traffic flow information%(Fig.~\ref{fig:NYCC_Estimate})
It was previously observed from Fig.~\ref{fig:UDDS_T_bat_SingleLayer_MPC_LongH_resize} that the single-layer MPC with exact vehicle peed profile results in up to $5\%$ saving in the battery energy compared to the rule-based controller. On the other hand, up to $3.9\%$ energy saving is achieved when using traffic flow information, compared to 5\% with the exact speed profile. Despite the mismatch between the real vehicle speed profile and long range prediction of the vehicle speed profile based on the traffic flow information, the energy saving is still substantial. Thus, the estimated long range vehicle speed profile via the traffic flow speed data can serve the purpose of the BTM system optimization.~%(Fig.~\ref{fig:NYCC_Estimate}), given the relatively slow dynamics of the thermal system, the average estimate of the traffic flow speed over the long horizon can serve the purpose of the BTM system optimization. On the other side, it can be seen that the results of $T_{bat}$ control is different. In both cases, the battery temperature is enforced to remain under the limit. However, 
At the same time, the single-layer MPC using the exact vehicle speed profile results in less frequent constraint violation (by 74\%) and lower average battery temperature (by 4\%), compared to that using vehicle speed profile based on traffic flow information.%with the single-Layer MPC with average traffic floe seed data. 
\vspace{-0.15cm} 

\section{Two-Layer MPC for Battery Thermal and Energy Optimization} \label{sec:TwoMPC} \vspace{-0.1cm} 

It was shown that the traffic flow information over a long horizon can be used for battery thermal and energy management optimization. However, the computational burden is still considerable. Fig.~\ref{fig:UDDS_T_bat_LongH_SingleLayer_SecondLayer_180} shows the CPU computation time per iteration for the single-layer MPC, and it can be seen that while the sampling time is $1~sec$, the maximum computation time can reach as much as $20~sec$, even on a powerful Core i7@2.60 GHz processor. In order to leverage the energy saving potentials of the long horizon traffic flow information and reduce the computation time of the MPC, we propose a two-layer MPC for battery thermal and energy optimization with a scheduling layer and a piloting layer as illustrated in Fig.~\ref{fig:TwoLayer_MPC_Schematic}. The scheduling layer has a relatively long horizon ($H_l$), and the dynamic of the system is sampled at a slower rate ($T_l>T_s$). The piloting layer has a short prediction horizon $H_s$, with a sampling time of $T_s$.\vspace{-0.15cm} 
%
\begin{figure}[t!]
	\begin{center}
		\includegraphics[width=7.7 cm]{Results/TwoLayer_MPC_Schematic.eps} \vspace{-0.35cm}   
		\caption{Schematic of Two-Layer NMPC for battery thermal and power management optimization.}\vspace{-0.85cm} 
		\label{fig:TwoLayer_MPC_Schematic} 
	\end{center}
\end{figure}
%

\subsection{Scheduling Layer MPC with Long Horizon}
%
In order to make the long-horizon MPC computationally efficient, the dynamic models for $\dot{T}_{bat}$ and $\dot{SOC}$ are simplified. To this end, first, $I_{bat}$ equation from (\ref{eqn:Eq4}) is approximated by using the Taylor series expansion with different accuracies for $SOC$ ($I_{bat,SOC}$), and the current ($I_{bat,T_{bat}}$)~\cite{bauer2014thermal}: 
%

\vspace{-0.35cm} 
\small
\begin{gather}
\label{eqn:Eq12}
I_{bat,SOC}(t)=\frac{a_c\dot{Q}+P_{trac}}{U_{oc}}+\frac{R_{bat}(a_c\dot{Q}+P_{trac})^2}{U_{oc}^3},
\end{gather}
%
\vspace{-0.5cm} 
% 
\begin{gather}
\label{eqn:Eq13}
I_{bat,T_{bat}}(t)=\frac{a_c\dot{Q}+P_{trac}}{U_{oc}}.
\end{gather}
\normalsize
%
%\doublespacing
%
Next, Eqs.~(\ref{eqn:Eq12}) and (\ref{eqn:Eq13}) are used to re-write the discretized battery state-of-charge ($f_{SOC,l}$) and temperature ($f_{T_{bat},l}$) dynamics over the long horizon $H_l$ assuming the sampling time $T_l$:  
%

\vspace{-0.85cm} 
\small
\begin{gather}
\label{eqn:Eq{14}}
{SOC}_{l}(k+1)={SOC}_{l}(k)+~~~~~~~~~~~\\
T_l\Big(\frac{R_{bat}(a_c\dot{Q}+P_{trac})^2+U_{oc}^2(a_c\dot{Q}+P_{trac})}{C_{nom}U_{oc}^3}\Big), \nonumber
\end{gather}
%
\vspace{-0.5cm} 
%
\begin{gather}
\label{eqn:Eq{15}}
{T}_{bat,l}(k+1)={T}_{bat,l}(k)+~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~\\
T_l\Big(\frac{\dot{Q}(2a_cR_{bat}P_{trac}+U_{oc}^2)+R_{bat}P_{trac}^2}{C_{th, bat}U_{oc}^2}\Big) \nonumber
\end{gather}
\normalsize
%
where $SOC_l$ and $T_{bat,l}$ designate the states of the simplified model used in the scheduling layer. The scheduling layer MPC is based on the following optimization problem formulation: \vspace{-0.25cm} 
%-------------------------------------
\begin{gather} \label{eqn:Eq16}
\begin{aligned}
& \underset{\dot{Q}(\cdot|k)}{\text{min}} & & \sum_{i=0}^{H_l} P_{temp}(i|k),  \\
%\tilde{\boldsymbol{y}}(k) & \\
& \text{s.t.}
& & T_{bat,l}(i+1|k)=f_{T_{bat},l}(i|k),~{ i=0,\cdots,H_l},\\
& 
& & SOC_l(i+1|k)=f_{SOC,l}(i|k),~{ i=0,\cdots,H_l},\\
& 
& &T_{bat}^{LL}\leq T_{bat,l}(i|k) \leq T_{bat}^{UL},~{ i=0,\cdots,H_l},\\
& 
& &30\% \leq SOC_l(i|k)\leq 90\%,~{ i=0,\cdots,H_l},\\
% \end{aligned} 
% \end{gather}
% %
% \begin{gather} \label{eqn:Eq16}
% \begin{aligned}
% & 
% & &T_{bat}^{LL}\leq T_{bat,l}(i|k) \leq T_{bat}^{UL},~{ i=0,\cdots,H_l},\\
% & 
% & &30\% \leq SOC_l(i|k)\leq 90\%,~{ i=0,\cdots,H_l},\\
& 
& &-50~W\leq\dot{Q}(i|k)\leq 0,~{ i=0,\cdots,H_l-1},\\
& 
& & T_{bat,l}(0|k)=T_{bat}(k),~SOC_l(0|k)=SOC(k).%\\
%& 
%& & \dot{Q}^*(0|k)=\dot{Q}(k)   %\vspace{-0.5cm}
\end{aligned} 
\end{gather}
%--------------------------------------
The scheduling layer MPC optimizes $\dot{Q}$ over the long horizon $H_l$, and the solution ($\dot{Q}^*$) is used to schedule the desired values of the battery temperature ($T_{bat}^*$) and state-of-charge ($SOC^*$) for the piloting layer. Note that the structure of the scheduling layer MPC is similar to the single-layer MPC in Eq.~(\ref{eqn:Eq11}), but with a different sampling rate. This results in significantly reduced computational load, as will be shown later. %However, as it will be shown later, the MPC of the scheduling layer is computationally faster than the single-layer MPC.%, and (iii) the demanded traction power profile, which is estimated with respect to the average traffic flow speed (fig.~\ref{fig:NYCC_Estimate}), has a significantly more smooth shape than the actual traction power profile used by the Single-Layer MPC; thus, the solver spends less time to find the solution of the optimization problem. 

\vspace{-0.2cm}
\subsection{Piloting Layer MPC with Short Horizon}
%
$T_{bat}^*$ and $SOC^*$ from the scheduling layer are passed on to the piloting layer, where these values are used by a short-horizon MPC for tracking. The output of the scheduling layer MPC is updated every $T_l$, during which the output of the short-horizon MPC is updated $T_l/T_s$ times. %Let $\xi\in \mathbb{Z}$ be the ratio between the long and short horizon length ($\xi=H_l/H_s$). 
The length of the scheduled values which need to be passed on to the piloting layer depends on the piloting layer prediction horizon ($H_s$). Moreover, since $T_l>T_s$, the scheduled $T_{bat}^*$ and $SOC^*$ are passed on as piece-wise functions: $T_{bat}^*(t|k)$ and $SOC^*(t|k)$~\cite{lefort2013hierarchical}. %This means that the reference trajectories passed to the piloting layer are assumed to be constant over a $\xi.T_s~sec$ period. 
Fig.~\ref{fig:Task5_Integrated_HVAC_BTM} shows the communication process between the two layers, and how the scheduled references are passed on to the piloting layer from the scheduling layer. %\vspace{-0.5cm} 
%

The short-horizon MPC of the piloting layer is formulated as follows to track the scheduled $T_{bat}^*$ and $SOC^*$ references from the scheduling layer: \vspace{-0.25cm} 
%-------------------------------------
\begin{gather} %\label{eqn:Eq{17}}
\begin{aligned}
& \underset{\dot{Q}(\cdot|k)}{\text{min}} & & \sum_{j=0}^{H_s} \left\lbrace\Big((T_{bat}(j|k)-T_{bat}^*(j|k)\Big)^2 \right.\\
& 
& &\left.~~~~~+w_1\big(SOC(j|k)-SOC^*(j|k)\Big)^2 \right\rbrace, \nonumber%\\
\end{aligned}
\end{gather}
%
\begin{gather} \label{eqn:Eq{17}}
\begin{aligned}
%\tilde{\boldsymbol{y}}(k) & \\
& \text{s.t.}
& & T_{bat}(j+1|k)=f_{T_{bat}}(j|k),~{ j=0,\cdots,H_s},\\
& 
& & SOC(j+1|k)=f_{SOC}(j|k),~{ j=0,\cdots,H_s},\\
%& 
%& &T_{bat}(i|k)\in\mathcal{T},~SOC(i|k)\in\mathcal{SOC},~{\scriptstyle i=0,\cdots,H_l}\\
& 
& &-50~W\leq\dot{Q}(j|k)\leq 0,~{ j=0,\cdots,H_s-1},\\
& 
& & T_{bat}(0|k)=T_{bat}(k),~SOC(0|k)=SOC(k).%\\
%& 
%& & \dot{Q}(0|k)=\dot{Q}(k)
\end{aligned}
\end{gather}
%--------------------------------------
\vspace{-0.35cm} 
\begin{figure}[h!]
 	\begin{center}
 		\includegraphics[width=7.8 cm]{Results/TwoLayer_MPC_Block_Schematic_v2.eps} \vspace{-0.35cm}   % The printed column width is 8.4 cm.
 		\caption{Two-layer hierarchical structure scheme. The calculated $T_{bat}^{*}$ and $SOC^{*}$ references are sent in a block form from the scheduling layer to the piloting layer, where the short-horizon NMPC tracks these references.}\vspace{-0.75cm} 
 		\label{fig:Task5_Integrated_HVAC_BTM} 
\end{center}
\end{figure}

When performing optimization in the piloting layer, we assume that the vehicle speed and the demanded traction power can be estimated accurately over the short horizon. Moreover, the constraints on the battery temperature and $SOC$ are not considered, as the long-horizon MPC has enforced these constraints in the scheduling layer. This will help to (i) reduce the computation time of the piloting layer optimization problem, (ii) avoid the infeasibility problem of the short-horizon MPC.

%In this study, the long-horizon MPC of the scheduling layer has a prediction horizon of $H_l=50$ ($250~sec$) and, the short-horizon MPC runs with $H_s=10$ (10~sec). (\blueline) 
{The energy saving result and computation times of the two-layer MPC are also compared with the single-layer MPC in Fig.~\ref{fig:UDDS_T_bat_LongH_SingleLayer_SecondLayer_180}. Using the same traffic flow information for both two-layer (\blueline) and single-layer (\redline) MPCs, the comparison results show that the energy saving potentials from both MPCs are the same $3.9\%$ improvement compared to the baseline. Moreover, the computation times of the two-layer MPC at both layers are significantly lower than the single-layer MPC, because of: 
%
\begin{itemize}
\item The larger sampling time used at the scheduling layer leading to substantially reduced optimization variables for the same prediction time window. %time length of the prediction horizon, the scheduling layer MPC deals with less optimization variables.
%
\item Simplified dynamics of $SOC_l$ and $T_{bat,l}$.
%
\item Non-redundant constraint enforcement with the battery temperature constraint being enforced at the scheduling layer and removed from the piloting layer MPC. %Since $T_{bat}$ is regulated to be very close to $T_{bat}^{UL}$ to save energy, the solver of the single-layer MPC spends more time to enforce $T_{bat}^{UL}$ constraint. On the other side, for the short-horizon MPC of the piloting layer, while the temperature is close to $T_{bat}^{UL}$, since there is no constraint on $T_{bat}$, the optimization problem just for tracking $SOC^*$ and $T_{bat}^*$ can be solved much faster.
\end{itemize}
}\vspace{-0.2cm} 

\subsection{Intelligent Online Constraint Handling}

Since the battery temperature constraint is removed from the short-horizon MPC, an intelligent online constraint handling (IOCH) algorithm is added to the structure of the two-layer MPC (shown in Fig.~\ref{fig:TwoLayer_MPC_Schematic}) to reduce the battery temperature limit violation that may be caused by the mismatch between the actual driving conditions and assumed driving conditions based on average traffic flow information. The IOCH block takes into account the violation of the battery temperature limits, and monitors the difference between $T_{bat}$ and $T_{bat}^*$. The addition of the IOCH block introduces an extra optimization variable $\epsilon$ which modifies the upper temperature bound at the scheduling layer to avoid temperature limit violations at the piloting layer, with consideration of the battery cooling power minimization. For this purpose, the cost function of the long-horizon MPC at the scheduling layer in Eq.~(\ref{eqn:Eq16}) is modified as follows: \vspace{-0.25cm}
%
\begin{gather}
\label{eqn:Eq18}
\begin{aligned}
& \underset{\dot{Q}(i|k),\epsilon(k)}{\text{min}} & & \sum_{i=0}^{H_l} P_{temp}(i|k)+\gamma(\delta(T_{bat},T_{bat}^{UL})-\epsilon(i|k))^2,
\end{aligned}
\end{gather}
%
where, $\gamma$ is a weighting factor to adjust the controller effort for reducing the constraint violation. The long-horizon MPC is subject to the constraints listed in (\ref{eqn:Eq16}), except for $T_{bat}(i|k)$, which is now subject to: \vspace{-0.15cm}
%
\begin{gather}
\label{eqn:Eq19}
T_{bat}^{UL}(i|k)\leq T_{bat}^{UL}-\epsilon(i|k),~{ i=0,\cdots,H_l}\\
\epsilon(i|k)\geq 0,~{ i=0,\cdots,H_l-1}, \nonumber
\end{gather}
%
where, $T_{bat}^{UL}(i|k)$ denotes the variable upper limit of the battery temperature operation. The function $\delta(T_{bat},T_{bat}^*)$ in Eq.~(\ref{eqn:Eq18}) is defined as follows: %\vspace{-0.1cm}
%
\begin{gather}
\label{eqn:Eq20}
\delta(T_{bat},T_{bat}^{UL})=\begin{cases}
0 & if~ T_{bat}\leq T_{bat}^{UL}\\
T_{bat}-T_{bat}^{UL}  & if~ T_{bat}>T_{bat}^{UL}
\end{cases}
\end{gather}
%
Fig.~%\ref{fig:UDSS_T_bat_TwoLayer} and 
\ref{fig:UDDS_T_bat_TwoLayer_ini39_V2} shows the performance of the two-layer MPC for UDDS at $T_{bat,0}=39^oC$. It can be seen that when $T_{bat}^{UL}$ is constant and set to be $40^oC$, the scheduled battery temperature trajectory ($T_{bat}^*$) does not violate the upper limit constraint. But, the actual battery temperature does because of the mismatch between the real driving cycle and the traffic flow velocity prediction. However, by using Eq.~(\ref{eqn:Eq18}) as the cost function of the scheduling layer MPC, the added optimization variable $\epsilon$ modifies the upper limit (Eq.~(\ref{eqn:Eq19})) with respect to the mismatches between $V_{flow}$ and $V_{veh}$, and reduces the overall $T_{bat}^{UL}$ violation by $13\%$. The impact of the addition optimization variable $\epsilon$ on the two-layer MPC computation time will be discussed in the next section.%Sec.~\ref{sec:4}. %As discussed before, these mismatches often occur during sharp accelerations and deceleration events, where the average traffic flow speed information does not reflect those aggressive moments. 
\vspace{-0.3cm} 
%
\begin{figure}[h!]
	\begin{center}
		\includegraphics[width=8.2 cm]{Results/UDDS_T_bat_TwoLayer_T039_resize_v3.eps} \vspace{-0.4cm}   % The printed column width is 8.4 cm.
		\caption{The results of battery thermal management from Two-Layer MPC with and without IOCH for the UDDS ($T_{bat}^{UL}$=$40^oC$,~$T_{bat,0}$=$39^oC$).}\vspace{-0.7cm} 
		\label{fig:UDDS_T_bat_TwoLayer_ini39_V2} 
	\end{center}
\end{figure}
%
%The effectiveness of the proposed constraint handling technique, and its impact on the Two-Layer MPC computation time will be further discussed in Section~\ref{sec:4}.

\section{Two-Layer MPC Simulation Results }\label{sec:4}
%
% \begin{figure}[b]\vspace{-0.35cm}
% 	\begin{center}
% 		\includegraphics[width=\columnwidth]{Results/UDDS_T_bat_TwoLayer_T035_resize.eps} \vspace{-0.7cm}   % The printed column width is 8.4 cm.
% 		\caption{The results of battery thermal management by using the two-layer NMPC, simple economy MPC, and On/Off controllers for the EPA Urban Dynamometer Driving Schedule (UDDS) ($T_{bat}^{UL}=40^oC$,~$T_{bat,0}=35^oC$).}\vspace{-0.35cm} 
% 		\label{fig:UDSS_T_bat_TwoLayer} 
% 	\end{center}
% \end{figure}
%
%
%In this section, the proposed Two-Layer MPC is designed and simulated for battery and energy management optimization of an electric vehicle described in Section~\ref{sec:1}. 
%
% \begin{figure}[h!]
% 	\begin{center}
% 		\includegraphics[width=\columnwidth]{Results/UDDS_SOC_TwoLayer.eps} \vspace{-0.7cm}   % The printed column width is 8.4 cm.
% 		\caption{The results of battery power management by using the two-layer NMPC, simple economy MPC, and On/Off controllers for the EPA UDDS ($T_{bat}^{UL}=40^oC$,~$T_{bat,0}=35^oC$).}\vspace{-0.3cm} 
% 		\label{fig:UDDS_SOC_TwoLayer} 
% 	\end{center}
% \end{figure}
%
% \begin{figure}[h!]
% 	\begin{center}
% 		\includegraphics[width=\columnwidth]{Results/UDDS_SOC_TwoLayer_ini39.eps} \vspace{-0.7cm}   % The printed column width is 8.4 cm.
% 		\caption{The results of battery power management by using the two-layer NMPC, simple economy MPC, and On/Off controllers for the EPA UDDS ($T_{bat}^{UL}=40^oC$,~$T_{bat,0}=39^oC$).}\vspace{-0.3cm} 
% 		\label{fig:UDDS_SOC_TwoLayer_ini39} 
% 	\end{center}
% \end{figure}

% It can be seen from Fig.%~\ref{fig:UDSS_T_bat_TwoLayer} and 
% ~\ref{fig:UDDS_T_bat_TwoLayer_ini39_V2} that the Two-Layer MPC with variable $T_{bat}^{UL}$ pushes down the battery temperature traces, which leads to overall reduction in violation of the target $40^oC$ upper limit. 
%Additionally, Fig.~\ref{fig:UDDS_T_bat_TwoLayer_ini39_V2} shows that when the initial battery temperature is close to the target upper limit, the Two-Layer MPC puts the efforts to cool down the battery at the early seconds, as it detects the major traction power demanding event downstream of the traffic flow, which becomes detectable by the controller via the long horizon of the scheduling layer.

% A similar simulation was carried out for the New York city Cycle (NYCC), which features low speed stop-and-go traffic conditions, and the results are shown in Fig.~\ref{fig:NYCC_T_bat_TwoLayer}. It is observed from Fig.~\ref{fig:NYCC_T_bat_TwoLayer} that at initial battery temperature of $39^0C$, the Two-Layer MPC with variable $T_{bat}^{UL}$ keeps $T_{bat}$ below the target upper limit for the entire driving cycle. On the other hand, the Two-Layer MPC with fixed $T_{bat}^{UL}$ shows some violation of the temperature constraints. Fig.~\ref{fig:NYCC_T_bat_TwoLayer} confirms the effectiveness of the modified cost function and constraints proposed in Eqs.~(\ref{eqn:Eq19}) and (\ref{eqn:Eq18}) in handling the constraint on the battery temperature, by compensating the mismatches between the real vehicle speed profile and the average traffic flow speed information at the scheduling layer. It should be mention that the simulation results show that while the Two-Layer MPC with variable $T_{bat}^{UL}$ makes the controller slightly more conservative with lower average battery temperature, the overall battery power consumption is not affected, and the final $SOC$ is the almost the same for the Two-Layer MPC with, and without variable $T_{bat}^{UL}$. This observation will be further discussed in the following.   %\vspace{-0.25cm}
% %
% \begin{figure}[t]
% 	\begin{center}
% 		\includegraphics[width=\columnwidth]{Results/NYCC_T_bat_TwoLayer.eps} \vspace{-0.7cm}   % The printed column width is 8.4 cm.
% 		\caption{The results of battery thermal management by using the two-layer NMPC, simple economy MPC, and On/Off controllers for the New York city cycle (NYCC) ($T_{bat}^{UL}=40^oC$,~$T_{bat,0}=39^oC$).}\vspace{-0.8cm} 
% 		\label{fig:NYCC_T_bat_TwoLayer} 
% 	\end{center}
% \end{figure}
%
% \begin{figure}[h!]
% 	\begin{center}
% 		\includegraphics[width=\columnwidth]{Results/NYCC_SOC_TwoLayer.eps} \vspace{-0.7cm}   % The printed column width is 8.4 cm.
% 		\caption{The results of battery power management by using the two-layer NMPC, simple economy MPC, and On/Off controllers for the New York city cycle (NYCC) ($T_{bat}^{UL}=40^oC$,~$T_{bat,0}=39^oC$).}\vspace{-0.3cm} 
% 		\label{fig:NYCC_SOC_TwoLayer} 
% 	\end{center}
% \end{figure}

%UDDS_T_bat_SingleLayer_MPC_Modified_Final_resize
In order to demonstrate the energy saving potentials of the proposed two-layer MPC for battery thermal management of electric vehicles, the predictive controller with IOCH is simulated for UDDS and the New York City Cycle (NYCC) at different initial battery temperature conditions. The NYCC features low speed stop-and-go traffic conditions. These results are compared with the traditional rule-based controller, and presented in Figs.~\ref{fig:UDDS_T_bat_SingleLayer_Tracking_Comparison}-\ref{fig:NYYC_SOC_SingleLayer_Tracking_Comparison}. Figs.~\ref{fig:UDDS_T_bat_SingleLayer_Tracking_Comparison} shows that despite $T_{bat}^{UL}$ violations during the period when demanding traction power occurs, the two-layer MPC brings back the temperature to below the target limit, and keeps the temperature close to this limit to minimize the required cooling power from the battery. It can be seen from Fig.~\ref{fig:UDDS_SOC_SingleLayer_Tracking_Comparison} that by the end of the driving cycle, the two-layer MPC reduces the drop in the battery $SOC$ by {$2.9\%$} and $2.8\%$ for $T_{bat,0}=35^oC$ and for $T_{bat,0}=39^oC$, respectively, compared to the rule-based controller. It should be noted from Fig.~\ref{fig:UDDS_SOC_SingleLayer_Tracking_Comparison} that compared to the two-layer MPC without IOCH, the energy saving results (as determined by terminal battery SOC) of the two-layer MPC with IOCH is $1\%$ lower, which is expected, as the overall battery temperature is lower and constraint violations are less frequent. This is the price paid for putting more effort to maintain $T_{bat}$ within the desired range. While temporary violations of $T_{bat}^{UL}$ is tolerated, it is required that $T_{bat}$ to be maintained withing the optimum operating range to improve the battery life and health in long term~\cite{zolot2002thermal}.\vspace{-0.15cm}
%
\begin{figure}[h!] %\vspace{-0.5cm}
	\begin{center}
		\includegraphics[width=8 cm]{Results/UDDS_T_bat_SingleLayer_MPC_Modified_Final_resize_v2.eps} \vspace{-0.4cm}   % The printed column width is 8.4 cm.
		\caption{The results of BTM by using Two-Layer MPC with IOCH and On/Off controller ($T_{bat}^{s.p.}$=$35^oC$) for UDDS at $T_{bat,0}$=$35^oC$ and $39^oC$.}\vspace{-0.5cm} 
		\label{fig:UDDS_T_bat_SingleLayer_Tracking_Comparison} 
	\end{center}
\end{figure}
%UDDS_SOC_SingleLayer_MPC_Modified_Final_resize_v3_addon
\begin{figure}[h!]
	\begin{center}
		\includegraphics[width=8 cm]{Results/UDDS_SOC_SingleLayer_MPC_Modified_Final_resize_v3.eps} \vspace{-0.05cm} \\
\includegraphics[width=8 cm]{Results/UDDS_SOC_SingleLayer_MPC_Modified_Final_resize_v3_addon.eps}\vspace{-0.4cm}   % The printed column width is 8.4 cm.
		\caption{The results of battery energy management by using Two-Layer MPC with IOCH and On/Off controller ($T_{bat}^{s.p.}$=$35^oC$) for UDDS at $T_{bat,0}$=$35^oC$ and $39^oC$.}\vspace{-0.75cm} 
		\label{fig:UDDS_SOC_SingleLayer_Tracking_Comparison} 
	\end{center}
\end{figure}
%
\begin{figure}[h!]
	\begin{center}
		\includegraphics[width=8 cm]{Results/NYCC_T_bat_SingleLayer_Tracking_Comparison_resize.eps} \vspace{-0.4cm}   % The printed column width is 8.4 cm.
		\caption{The results of BTM by using Two-Layer MPC with IOCH and On/Off controller ($T_{bat}^{s.p.}$=$35^oC$) for NYCC at $T_{bat,0}$=$35^oC$ and $39^oC$.}\vspace{-0.7cm} 
		\label{fig:NYYC_T_bat_SingleLayer_Tracking_Comparison} 
	\end{center}
\end{figure}

For the NYCC, since the vehicle speed is low on average, aggressive rises in the demanded traction power and battery temperature are not observed. Thus, the two-layer MPC is able to maintain the battery temperature well below the upper limit, even with $T_{bat,0}=39^oC$. By looking into the battery energy management results for the NYCC in Fig.~\ref{fig:NYYC_SOC_SingleLayer_Tracking_Comparison}, it can be seen that the conservative design of the rule-based controller results in a significant drop in the battery $SOC$ by the end of the driving cycle. Compared to the rule-based controller, the two-layer MPC reduces battery energy consumption (as determined by terminal $SOC$) by {$7.9\%$} and $7.7\%$ for $T_{bat,0}=39^oC$ and $T_{bat,0}=35^oC$, respectively. This is because the rule-based controller tries to maintain the temperature at $T_{bat}^{s.p.}=35^oC$, regardless of the traffic and driving conditions. %While the maximum demanded traction power during NYYC is lower than that of UDDS, the rule-based BTM demands for a relatively high tempering power. 
Unlike the rule-based controller, the two-layer MPC, which anticipates future vehicle speed profile based on the long-term traffic flow information, maintains $T_{bat}$ within the desired operation range, while minimizing the cooling power. %\vspace{-0.35cm}
%
%NYCC_SOC_SingleLayer_Tracking_Comparison_resize_v2_addon
\begin{figure}[h!]
	\begin{center}
\includegraphics[width=8 cm]{Results/NYCC_SOC_SingleLayer_Tracking_Comparison_resize_v2.eps} \\
\includegraphics[width=8 cm]{Results/NYCC_SOC_SingleLayer_Tracking_Comparison_resize_v2_addon.eps} \vspace{-0.4cm}   % The printed column width is 8.4 cm.
		\caption{The results of battery energy management by using Two-Layer MPC with IOCH and On/Off controller ($T_{bat}^{s.p.}$=$35^oC$) for NYCC at $T_{bat,0}$=$35^oC$ and $39^oC$.}\vspace{-0.55cm} 
		\label{fig:NYYC_SOC_SingleLayer_Tracking_Comparison} 
	\end{center}
\end{figure}
%

Table~\ref{tab:Computation_Time_Comparison_2} summarizes the average and maximum required computation times for each layer of the two-layer MPC with and without IOCH. It can be seen that the addition of the extra optimization variable $\epsilon$ to the cost function of the scheduling layer MPC increases the computation time by 142\%. Despite this increase, the average and maximum computation times of the scheduling layer MPC are less than the sampling time ($T_l$=$5~sec$). %Since the Two-Layer MPC with variable $T_{bat}^{UL}$ is keeping the battery temperature further away from the target upper limit,
Table~\ref{tab:Computation_Time_Comparison_2} also shows that the average computation time of the piloting layer MPC with IOCH is slightly reduced by $4\%$, compared to the same controller without IOCH. Moreover, it can be seen that in all cases, the average and maximum computation times of the piloting layer MPC is less than the sampling time $T_s$=$1~sec$. By comparing Table~\ref{tab:Computation_Time_Comparison_2} with Table~\ref{tab:Computation Time Comparison}, it can be observed that unlike the single-layer MPC, the two-layer MPC provides a computationally efficient framework, which allows for utilization of the long-term traffic information in the body of the electric vehicle battery thermal and energy management system in real-time. \vspace{-0.15cm} 
%
\begin{table}[h!]
%\linespread{0.8}
\begin{center}
\small
\centering 
\caption{Computation time comparison of the Two-Layer MPC with, and without variable $T_{bat}^{UL}$. 
\label{tab:Computation_Time_Comparison_2}} %\vspace{0.4cm}
\begin{tabular}{lcc}
        \hline\hline
\textcolor{blue}{Scheduling Layer MPC} & $T_{bat}^{UL}=40^oC$ & $T_{bat}^{UL}=variable$  \\ \hline
$~~~Average~CPU$      & 0.855 & 2.071  \\
$Time/Iteration~[sec]$ & \textcolor{red}{-} & \textcolor{red}{$\uparrow$142\%} \\\hline
%
$~~~max~CPU$      &  &    \\
$time/iteration~[sec]$ & 1.396 &4.265 \\
        \hline\hline
        %
\textcolor{blue}{Piloting Layer MPC} & $T_{bat}^{UL}=40^oC$ & $T_{bat}^{UL}=variable$  \\ \hline
$~~~Average~CPU$      & 0.206 & 0.197  \\
$Time/Iteration~[sec]$ & \textcolor{green}{-} & \textcolor{black!30!green}{$\downarrow$-4\%} \\\hline
%
$~~~max~CPU$      &  &    \\
$time/iteration~[sec]$ & 0.563 & 0.780 \\
        \hline\hline
    \end{tabular}
\end{center} \vspace{-0.55cm} 
\end{table}
\linespread{1}
%
%\vspace{-0.45cm}
% \begin{figure}[h!]
% 	\begin{center}
% 		\includegraphics[width=\columnwidth]{Results/UDDS_MPC_Tracking_Tbatdes30.eps} \vspace{-0.7cm}   % The printed column width is 8.4 cm.
% 		\caption{The results of battery thermal management by using the two-layer NMPC for tracking, and simple MPC for tracking for UDDS at $T_{bat,0}=35^oC$ for $T_{bat}^{s.p.}=30^oC$. }\vspace{-0.3cm} 
% 		\label{fig:UDDS_MPC_Tracking_Tbatdes30} 
% 	\end{center}
% \end{figure}
